Minimizing Quadratic Functions in Constant Time

A sampling-based optimization method for quadratic functions is proposed. Our method approximately solves the following $n$-dimensional quadratic minimization problem in constant time, which is independent of $n$: $z^*=\min_{\mathbf{v} \in \mathbb{R}^n}\langle\mathbf{v}, A \mathbf{v}\rangle + n\langle\mathbf{v}, \mathrm{diag}(\mathbf{d})\mathbf{v}\rangle + n\langle\mathbf{b}, \mathbf{v}\rangle$, where $A \in \mathbb{R}^{n \times n}$ is a matrix and $\mathbf{d},\mathbf{b} \in \mathbb{R}^n$ are vectors. Our theoretical analysis specifies the number of samples $k(\delta, \epsilon)$ such that the approximated solution $z$ satisfies $|z - z^*| = O(\epsilon n^2)$ with probability $1-\delta$. The empirical performance (accuracy and runtime) is positively confirmed by numerical experiments.

==> table/kernel_together.tex <==
\begin{tabular}{rrrrrrrrrr}
  \hline
method & k & $n=500$ & 1000 & 2000 & 5000 & $n=500$ & 1000 & 2000 & 5000 \\ 
  \hline
Proposed & 20 & $0.003\pm0.003$ & $0.001\pm0.001$ & $0.002\pm0.002$ & $0.002\pm0.002$ & $0.002$ & $0.002$ & $0.002$ & $0.002$ \\ 
  Proposed & 40 & $0.002\pm0.002$ & $0.001\pm0.001$ & $0.001\pm0.001$ & $0.001\pm0.002$ & $0.003$ & $0.003$ & $0.003$ & $0.003$ \\ 
  Proposed & 80 & $0.001\pm0.001$ & $0.000\pm0.000$ & $0.001\pm0.001$ & $0.001\pm0.002$ & $0.007$ & $0.007$ & $0.008$ & $0.008$ \\ 
  Proposed & 160 & $0.000\pm0.000$ & $0.000\pm0.000$ & $0.000\pm0.000$ & $0.000\pm0.000$ & $0.030$ & $0.030$ & $0.033$ & $0.035$ \\ 
  Nystr\"{o}m & 20 & $0.369\pm0.914$ & $1.301\pm2.450$ & $3.112\pm6.146$ & $0.699\pm0.964$ & $0.005$ & $0.012$ & $0.046$ & $0.274$ \\ 
  Nystr\"{o}m & 40 & $0.355\pm0.619$ & $0.421\pm0.702$ & $0.984\pm1.542$ & $0.374\pm0.666$ & $0.010$ & $0.022$ & $0.087$ & $0.513$ \\ 
  Nystr\"{o}m & 80 & $0.018\pm0.019$ & $0.040\pm0.047$ & $0.206\pm0.272$ & $0.571\pm0.792$ & $0.022$ & $0.049$ & $0.188$ & $0.942$ \\ 
  Nystr\"{o}m & 160 & $0.014\pm0.021$ & $0.035\pm0.054$ & $0.058\pm0.111$ & $0.025\pm0.028$ & $0.076$ & $0.116$ & $0.432$ & $1.972$ \\ 
   \hline
\end{tabular}

